Extremes of the 2d scale-inhomogeneous discrete Gaussian free field: Extremal process in the weakly correlated regime

We prove convergence of the full extremal process of the two-dimensional scale-inhomogeneous discrete Gaussian free field in the weak correlation regime. The scale-inhomogeneous discrete Gaussian free field is obtained from the 2d discrete Gaussian free field by modifying the variance through a function $\mathcal{I}:[0,1]\rightarrow [0,1]$. The limiting process is a cluster Cox process. The random intensity of the Cox process depends on the $\mathcal{I}^\prime(0)$ through a random measure $Y$ and on the $\mathcal{I}^\prime(1)$ through a constant $\beta$. We describe the cluster process, which only depends on $\mathcal{I}^\prime(1)$, as points of a standard 2d discrete Gaussian free field conditioned to be unusually high.

==> DGFF.tex <==
The most natural object to compare our results to is probably the DGFF $\{\phi^N_v\}_{v\in V_N}$.
In this case, we have 


==> abstract.tex <==
In this paper, we continue our research of the extreme values of the scale-dependent DGFF in 2d. In the case of weak correlations, i.e. strictly increasing variance parameters, we prove convergence of the extremal process of local extremes. The proof is be based on \cite{MR3433630}, where the authors prove the result for the DGFF. Our result is in line with those in the case of increasing speed BBM \cite{MR3351476}.

==> concentric_decomposition.tex <==
We have
\begin{align}
	\psi^N_{}
\end{align}

==> coupling_multiple_maxima.tex <==
In this section, we generalize the proof that gave us convergence of the centred maximum to a proof of the joint convergence of finitely many local maxima:
\begin{thm}
	Let $(A_1,\dotsc, A_l)$ be a collection of disjoint non-empty open subsets of $[0,1]^2$. Then,
	\begin{align}
		\left( \max\{\psi^N_v:v\in V_N, \, x/N\in A_k \}-m_N\right)_{k=1}^l
	\end{align}
	converges weakly as $N\rightarrow \infty$.
	\begin{[proof}
		The proof relies on a coupling of an auxiliary process and indepedent identically distributed random variables. This heavily uses the self-similarity of scales.
		We first want to fix notation: Let $K\in \mathbb{N}$, $\{w^K_i: \,i=1,\dotsc, K^2\}$ points enumerating $\{x/K:\, x\in \{0,\dotsc, K-1\}^2 \}$. If $N\in \mathbb{N}$ is such that it is divisible by $K$ and $\delta>0$ such that $\delta N/K\in \mathbb{N}$, we introduce the sets
		\begin{align}
			&V^{K,i}_N\coloneqq N w^K_i + V_{N/K}&\text{and}& V^{K,\delta,i}_N\coloneqq N w^K_i + (\delta N/K, (1-\delta )N/K)^2\cap \mathbb{Z}^2.
		\end{align} 
		Note, that the boxes $V^{K,i}_N$ are disjoint and that they tile $V_N$, i.e. $\cup_{i} V^{K,i}_N\cup \delta V^{K,i}_N \supset V_N \cup \delta V_N$.
		Also, let $V^{K,\delta}\coloneqq \cup_{i=1}^{K^2} V^{K,\delta,i}_N$. As we are passing to the continuum limit, we need the continuum analogue sets to the above, i.e. let $B^{K,i}\coloneqq w_i^K + (0,1/K)^2$ and set
		\begin{align}
			&B^{K,\delta,i }\coloneqq w^K_i +(\delta/K,(1-\delta )/K)^2 &\text{and} & B^{K,\delta}\coloneqq \cup_{i=1}^{K^2} B^{K,\delta,i}.
		\end{align}
		So Figure ... for an illustration.
		
		We need some constant $\beta_{K}$ and $\gamma(K)$ such that for $x\geq 0$ and all Borel $A\subset [0,1]^2$
		\begin{align}
			\mathbb{P}\left( =1\right)\coloneqq C \beta_Ke^{-2 \beta_K}\\
			\mathbb{P}\left(Y^K_i\geq x\right)\coloneqq \frac{\beta_k+x}{\beta_K}e^{-2x}\\
			\mathbb{P}\left(K(z^K_i-w^K_i)\in A\right)\coloneqq \int_A
		\end{align}
		the last should not play a role, as in our case the coarse field is constant in the considered subsets, thus the position of the local maxima is determined by the location of the maximizer of the fine field in the considered box.
		Next, we consider the some approximation of the sets $A_i$ by boxes, for which we have the correct right-tail asymptotic at hand.
		Further, we need some additional theorem, that states that the law of joint maxima over disjoint sets of the $(\sigma,\lambda)-$DGFF may be approximated by our 3-field decomposition of the field, that is we need to generalize the statement, which should be easily possible since we have the convergence of the correlations at macroscopic and microscopic distance. Thus the proof for this should just follow in the same way.
	\end{[proof}
\end{thm}


==> dist_invariance.tex <==
We first introduce necessary notation.
Let $\psi^\prime,\, \psi^{\prime \prime}$ be two independent copies of the scale-inhomogenoeus DGFF on $V_N$. Fix $t>0$, and set
\begin{align}
	\hat{\psi}^\prime \coloneqq \sqrt{1-\frac{t}{\log N}}\psi^\prime \quad \text{and}\quad \hat{\psi}^{\prime \prime}.
\end{align}
Then,
\begin{align}
	\psi\coloneqq \hat{\psi}^\prime +\hat{\psi}^{\prime \prime}
\end{align}
has the law of $\{\psi^N_v\}_{v\in V_N}$. Denote by $\Theta_{N,r}$ the set of $r-$local maxima, i.e. let
\begin{align}
	\Theta_{N,r} \coloneqq \{v\in V_N:\, \psi_v = \max_{u\in \Lambda_r(v)}\psi_u\}.
\end{align}

==> outlook.tex <==
Considering the fact, that in the case of the various speed BBM with strictly increasing variance, there is a complete description of the extremal process, including the clusters, and that there is strategy how to proof such things in the case of the DGFF by Marek and Oren, we think, that this should be a more or less simple adaptation. In particular, the cluster law should be given similarly by conditioning the process to stay below the local maximum. The main difficulty arises from this form of singular conditioning, as its probability vanishes in the limit. So, we have to make sure that it converges in the right sense. I think, that using our version of the Gibbs-Markov decomposition allows to define a concentric decomposition of the scale-dependent field, where one obtain a time-inhomogeneous random walk with decorations. This would allow to follow the path of Marek and Oren, using control variables etc., random walk estimates...
Here, we want to discuss, how we think we should approach the full extremal process. That is, we believe to be able to use the work from Marek and Oren. That is, to each local maximum, we want to attach a copy of a so-called cluster process, that now should look a bit different than in their paper, i.e. the scaled (with parameter $\sigma_M$) DGFF conditioned to be non-negative. The fact of the large variance parameter should affect the distance between two points, that is spacings should be larger.
Further, we could discuss that a similar approach in the case of general Gaussian log-correlated fields should be possible. In this case, similarly as done in this paper, we need to show additional extreme-point tightness. However, in this case there is nothing like the Gibbs-Markov property at hand, so we need to tackle this issue a bit differently. Further, the global position of local extremes should affect the random measure $Z(\mathrm{d}x)$ in this case. There might be even a slight dependence on the exact height of local maxima, between each other, that should be visible in the random measure.

==> proof_dist_inv.tex <==
Old stuff:In order to prove \autoref{thm:prob_dist_maximalparticles}, we have to show with high probability that there cannot be two vertices at ``intermediate distance'' to each other and both reaching an extremal height. We therefore study the sum of two vertices, under the additional restriction that their distance is ``intermediate''.
\begin{definition}
	Let $N\in \mathbbm{N}$, fix $r>1$ and define:
	\begin{align}
	\overset{\diamond}{\psi}_{N,r}&\coloneqq \max\{\psi_u^N+\psi_v^N:\,u,v \in V_N, \, r\leq \|u-v\|_2\leq \frac{N}{r} \},\\
	%\tilde{\psi}^{\diamond}_{N,r}&\coloneqq \max\{\psi^{4N}_{v+(2N,2N)}+\psi^{4N}_{u+(2N,2N)}: \, u,v \in V_N,\, r\leq %\|u-v\|_2\leq \frac{N}{r} \},\\
	\overset{\diamond}{S}_{N,r} &\coloneqq \max\{\tilde{S}_u^N +\tilde{S}_v^N:\,u,v\in V_N,\, r\leq \|u-v\|_2\leq \frac{N}{r} \}.\label{equation:5.3}
	\end{align}
\end{definition}
The following proposition relates $\overset{\diamond}{\psi}_{N,r}$ with $\overset{\diamond}{S}_{N,r}$.
\begin{comment}
The following lemma is based on a variant of Slepian's lemma (see \cite[Lemma~2.7]{MR3262484} and \cite[Lemma~2.9]{MR3262484}), and relates the maximum of the sum of particles from the scale-inhomogeneous DGFF with the maximum of the sum of particles from the IBRW.
\begin{lemma}\label{corollary:sudakov_fernique_sums}
For $N=2^n$, $n\in \mathbbm{N}$, let $\{\psi^N_v\}_{v\in V_N}$ be a scale-inhomogeneous DGFF and $\{R^N_v\}_{v\in V_N}$ the corresponding IBRW, as in \autoref{definition:ibrw}. For $p\in \mathbbm{N}$, define
\begin{align}
\mathcal{S}_{N,p}=\max\left\{\sum_{v\in A}\psi^N_v:\, |A|=p,\,A\subset V_N \right\}, \text{ and } \mathcal{R}_{N,p}=\max\left\{\sum_{v \in A} R^N_v:\,|A|=p,\,A\subset V_N \right\}.
\end{align}
Then, there is a constant $q\in \mathbbm{N}$ such that
\begin{align}
\mathbbm{E}\left[\mathcal{S}_{N,p} \right]\leq \mathbbm{E}\left[\mathcal{R}_{2^q N,p} \right].
\end{align}
\begin{proof}
Let $\tilde{R}^N_v=R^N_v+qX_v$, where $\{X_v\}_{v\in V_N}$ are i.i.d. standard Gaussian random variables, and define
\begin{align}
\mathcal{R}^{*}_{N,l}=\max\left\{\sum_{v \in A} \tilde{R}^N_v:\,|A|=l,\,A\subset V_N \right\}.
\end{align}
Note that each $A\subset V_N$ has a corresponding set $2^q A\subset V_{2^q N}$. On such sets, $\mathbb{E}\left[\tilde{R}^N_u \tilde{R}^N_v\right]\geq \mathbb{E}\left[R^{2^q N}_{2^q u} R^{2^q N}_{2^q v}\right]$, while variances match. Moreover, the maximum in $\mathcal{R}_{2^q N,p}$  is taken over a larger class of subsets than in $\mathcal{R}^{*}_{N,p}$, and thus, using Sudakov-Fernique,
\begin{align}
\mathbbm{E}\left[\mathcal{R}^{*}_{N,p} \right]\leq \mathbbm{E}\left[\mathcal{R}_{2^q N,p} \right].
\end{align}
Let $\{\tilde{\psi}^{N}_{v}\}_{v\in V_{4N}}$ be another centred Gaussian field, defined as
\begin{align}\label{equation:5.8}
\tilde{\psi}^N_v= \psi^N_v +\sigma_1 \mathbb{E}\left[\phi^{4N}_v|\sigma\left(\phi^{4N}_w:w\notin (2N,2N)+V_N\right)\right],\quad \text{for } v\in V_{4N},
\end{align}
where $\psi^N_v=0$, for $v\notin (2N,2N)+V_N$ and where $\{\phi^{4N}_v\}_{v\in V_{4N}}$ is a DGFF on $V_{4N}$, independent of $\{\psi^N_v\}_{v\in (2N,2N)+V_N}$.
Let $X$ be another independent standard Gaussian random variable. After possibly increasing the constant $q$, we can choose a non-negative sequence, $\{a_v\}_{v\in (2N,2N)+V_N}$, such that, for any $v\in (2N,2N)+V_N$,
\begin{align}
&\mathrm{Var}\left(\tilde{\psi}^{N}_v+a_v X \right)=\mathrm{Var}\left(\tilde{R}^N_v \right).
\end{align}
By \autoref{lemma:cov_comp} $i.$ and $iii.$, there is a constant $C>0$ such that $|a_u-a_v|\leq C$.
Moreover, let
\begin{align}
\mathcal{S}^{*}_{N,p}=\max \left\{\sum_{v\in A} \tilde{\psi}^{N}_v+a_vX:\,|A|=p,\,A\subset V_N \right\}.
\end{align}
As $\tilde{\psi}^N_v$ is a sum of two independent centred Gaussian fields (cp. \eqref{equation:5.8}), Sudakov-Fernique implies
\begin{align}
\mathbbm{E}\left[\mathcal{S}_{N,p} \right]\leq \mathbbm{E}\left[\mathcal{S}^{*}_{N,p} \right].
\end{align}
Choosing $q=4C$, and using \autoref{lemma:cov_comp} $i.$ and $iii.$, it follows that, for all $u,v \in V_N$,
\begin{align}
\mathbbm{E}\left[\tilde{R}^N_u \tilde{R}^N_v \right]\leq \mathbbm{E}\left[\left(\tilde{\psi}^{N}_{u+(2N,2N)}  +a_{u+(2N,2N)}X\right)\left(\tilde{\psi}^{N}_{v+(2N,2N)}  +a_{v+(2N,2N)}X \right) \right].
\end{align}
Thus, one can apply \cite[Lemma~2.7]{MR3262484} and conclude the proof of \autoref{corollary:sudakov_fernique_sums}.
\end{proof}
\end{lemma}
\end{comment}

\begin{prop}\label{proposition:comparison_to_maxsum_MIBRW}
	There is a constant $\kappa\in \mathbbm{N}$, such that, for all $r,n \geq \kappa$ and $N=2^n$,
	\begin{align}\label{eq:proposition_comparison_to_maxsum_MIBRW}
	\mathbbm{E}\left[\overset{\diamond}{S}_{2^{-\kappa}N,r} \right]\overset{}{\leq} \mathbbm{E}\left[\overset{\diamond}{\psi}_{N,r} \right] \overset{}{\leq} \mathbbm{E}\left[\overset{\diamond}{S}_{2^\kappa N,r}\right].
	\end{align}
	\begin{proof}
		We start with the proof of the lower bound.
		By \autoref{lemma:cov_comp} $iii.$, there is a constant $\alpha>0$, such that, for any $u,v\in V_{2^{-\kappa-1}N}$, $\left|\mathrm{Var}\left[\tilde{S}^{N/2}_{2^\kappa u}\right]-\mathrm{Var}\left[\psi^N_{2^\kappa u +(\frac{N}{2},\frac{N}{2})}\right]\right|\leq \alpha$. By construction, $\mathrm{Var}\left[\tilde{S}^{2^{-\kappa-1}N}_u\right]=\log(2)(n-\kappa-1)$, i.e. the variance decreases linearly in $\kappa$ when keeping $N$ fixed, whereas by \autoref{lemma:convergence_cov_neardiag_offdiag} $i.$  $\mathrm{Var}\left[\psi^N_{2^\kappa u +(\frac{N}{2},\frac{N}{2})}\right]=\log(2)n+O(1)$.
		Moreover, when $\kappa\ll N$, \autoref{lemma:cov_comp} $iii.$ implies
		\begin{align}\label{equation:5.14}
		\left|\mathbb{E}\left[\tilde{S}^{2^{-\kappa-1}N}_u \tilde{S}^{2^{-\kappa-1}N}_v\right] - \mathbb{E}\left[\psi^N_{2^\kappa u +(\frac{N}{2},\frac{N}{2})}\psi^N_{2^\kappa v +(\frac{N}{2},\frac{N}{2})}\right]\right| \leq C.
		\end{align}
		Using \eqref{equation:5.14} , and as the $\mathrm{Var}\left[\tilde{S}^{2^{-\kappa-1}N}_u\right]$ decays in $\kappa$, one can choose $\kappa$ sufficiently large, independent of $N$, and such that
		\begin{align}\label{equation:5.15}
		\mathbb{E}\left[\left(\tilde{S}^{2^{-\kappa}N}_u-\tilde{S}^{2^{-\kappa}N}_v \right)^2 \right]\leq \mathbb{E}\left[\left(\psi^N_{2^\kappa u +(\frac{N}{4},\frac{N}{4})}- \psi^N_{2^\kappa v +(\frac{N}{4},\frac{N}{4})}\right)^2 \right].
		\end{align}
		The first inequality in \eqref{eq:proposition_comparison_to_maxsum_MIBRW} now follows from \eqref{equation:5.15} using \cite[Lemma~2.7]{MR3262484}, a variant of Slepian's lemma for sums.
		To prove the upper bound in \eqref{eq:proposition_comparison_to_maxsum_MIBRW}, we argue similarly.
		On the one hand, using \autoref{lemma:cov_comp} $i.$, it holds that $\mathrm{Var}\left[\tilde{S}^{2^\kappa N}_{2^\kappa u}\right]=\log(2)(n+\kappa)$, while at the same time, $\mathbb{E}\left[\tilde{S}^{2^\kappa N}_{2^\kappa u}\tilde{S}^{2^\kappa N}_{2^\kappa v}\right]=\log(2)(n+\kappa)\mathcal{I}_{\sigma^2}\left(\frac{d^N(v,w)}{n+\kappa}\right)+O(1)$. Thus, while the variance increases linearly in $\kappa$, the covariance may vary only up to uniformly bounded constants, as $n\rightarrow \infty$.
		Thus, noting that $r\leq \|u-v\|_2 \leq \frac{N}{r}$ implies $r\leq 2^\kappa \|u-v\|_2\leq \frac{2^\kappa N}{r}$, and using \autoref{lemma:cov_comp} $iii.$, one gets for $\kappa$ chosen large enough and independent of $N$,
		\begin{align}\label{equation:4..6}
		\mathbb{E}\left[\left(\psi^{4N}_{u+(2N,2N)}- \psi^{4N}_{v+(2N,2N)}\right)^2 \right] \leq \mathbb{E}\left[\left(\tilde{S}^{2^\kappa N}_{2^\kappa u}- \tilde{S}^{2^\kappa N}_{2^\kappa v}\right)^2 \right]=2\log (2)(n+\kappa)\mathcal{I}_{\sigma^2}\left(\frac{d^N(v,w)}{n+\kappa}\right)+O_\kappa(1).
		\end{align}
		Moreover, by the Gibbs-Markov property of the DGFF, there is a constant $C>0$ such that
		\begin{align}\label{equation:4..7}
		\mathbb{E}\left[\left(\psi^N_u-\psi^N_v\right)^2\right] \leq \mathbb{E}\left[\left(\psi^{4N}_{u+(2N,2N)}- \psi^{4N}_{v+(N,N)}\right)^2 \right]+C.
		\end{align}
		Increasing $\kappa$, increases the right-hand side in \eqref{equation:4..6} linearily in $\kappa$, while \eqref{equation:4..7} is independent of $\kappa$. This allows to apply \cite[Lemma~2.7]{MR3262484}, which implies the second inequality in \eqref{eq:proposition_comparison_to_maxsum_MIBRW}. This concludes the proof of \autoref{proposition:comparison_to_maxsum_MIBRW}.
	\end{proof}
\end{prop}
\autoref{proposition:comparison_to_maxsum_MIBRW} reduces the proof of suitable upper and lower bounds for $\mathbbm{E}\left[\overset{\diamond}{\psi}_{N,r} \right]$ to upper and lower bounds for $\mathbbm{E}\left[\overset{\diamond}{S}_{N,r}\right]$. While the first is associated to the scale-inhomogeneous DGFF, the latter involves only the MIBRW, which is easier to analyze. The following lemma provides suitable upper and lower bounds for $\mathbbm{E}\left[\overset{\diamond}{S}_{N,r}\right]$.
\begin{lemma}\label{lemma:boundonexpofsumofmbrw}
	There are constants $C,c_1,c_2>0,$ so that
	\begin{align}
	2 m_n -c_2 \log\log r \leq \mathbbm{E}\left[\overset{\diamond}{S}_{N,r}\right]\leq 2 m_n - c_1 \log\log r +C.
	\end{align}
\end{lemma} 
We split the proof into upper and lower bound. We start with results used in the proof of the upper bound, which we reduce further, by Gaussian comparison, to an upper bound of a sum of two particles of a IBRW. By Gaussian comparison and since we have $\mathcal{I}_{\sigma^2}(x)<x$, for $x\in (0,1)$, one sees that, in order to obtain an upper bound in \autoref{lemma:boundonexpofsumofmbrw}, it suffices to consider a two-speed branching random walk, $(X^N_v(j))_{v\in V_N, 0\leq j \leq n}$. Choose the first speed to be $0$ and the second to be $\sigma_{max}^2$, where $\sigma_{max}=\text{ess} \sup\{ \sigma(s):0\leq s\leq 1\}$. To match variances, the change of speed occurs at scale $1-1/\sigma_{max}^2$. Indeed, as the distance on the tree is, up to an additional constant, smaller than the logarithm of the distance on the torus, there is some $\kappa\in \mathbb{N}$ and an independent centred Gaussian $G$, whose variance grows linearly in $\kappa$, such that for any $N\in \mathbb{N}$, $N$ sufficiently large, and any $v\in V_N$,
\begin{align}\label{equation:5.38}
\mathbbm{E}\left[\left(X^{2^\kappa N}_{2^\kappa u}-X^{2^\kappa N}_{2^\kappa v}\right)^2\right]\geq \mathbbm{E}\left[\left((\tilde{S}^N_u+G)-(\tilde{S}^N_v+G)\right)^2\right].
\end{align}
\eqref{equation:5.38} allows to apply \cite[Lemma~2.7]{MR3262484}, which reduces the proof of the upper bound in \autoref{lemma:boundonexpofsumofmbrw} to prove a suitable upper bound for $\mathbb{E}\left[\max_{u\sim_s v,s\in[\log r,n- \log r]} X^N_u+X^N_v \right]$, which is done next.
\begin{comment}
For the following, let $\lambda= 1/\sigma_{max}^2$. We use the IBRW as defined above, denoted by $(X^N_v(j))_{v\in V_N, 0\leq j \leq n}$, in \autoref{proposition:8.2}, \autoref{corollary:upbound_prob_maxsum_BRW} and in the proof of \autoref{lemma:boundonexpofsumofmbrw}. First, we make the following observation:
Let $X^{*,\prime}_N, X^{*}_N$ be two independent copies of maxima of such IBRWs. For any $n\in \mathbb{N}$ and $y\geq 0$,
\begin{align}\label{equation:tail_sum_IBRW}
\mathbb{P}\left(X^{*}_{N}+X^{*,\prime}_{N}\geq 2 m_n+2y\right)
&\leq \sum_{j\in \mathbb{Z}}\mathbb{P}\left(X^{*}_{N}-m_n\in[j,j+1)\right)\mathbb{P}\left(X^{*,\prime}_{N}\geq m_n+2y-(j+1)\right).
\end{align}
Note that, by symmetry, we have both
\begin{align}\label{equation:5.20}
&\sum_{j\geq 2y} \mathbb{P}\left(X^{*}_{N}-m_n\in[j,j+1)\right)\mathbb{P}\left(X^{*,\prime}_{N}\geq m_n+2y-(j+1)\right)\nonumber\\
&\qquad\qquad\qquad\qquad = \sum_{j<0}\mathbb{P}\left(X^{*}_{N}-m_n\in[j,j+1)\right)\mathbb{P}\left(X^{*,\prime}_{N}\geq m_n+2y-(j+1)\right),
\end{align}
and
\begin{align}\label{equation:5.19}
\sum_{j<0}\mathbb{P}\left(X^{*}_{N}-m_n\in[j,j+1)\right)\mathbb{P}\left(X^{*,\prime}_{N}\geq m_n+2y-(j+1)\right)& \leq \mathbb{P}\left(X^{*}_N\leq m_n\right)\mathbb{P}\left(X^{*,\prime}_{N}\geq m_n+2y\right)\nonumber\\
&\leq\mathbb{P}\left(X^{*,\prime}_{N}\geq m_n+2y\right).
\end{align}
We use \cite[Theorem 4.1]{MR3361256}, which in our case becomes
\begin{align}\label{equation:bound_tail_IBRW}
ce^{-2y}\leq \mathbbm{P}\left(X^{*}_N\geq m_n+y\right)\leq C(1+y)e^{-2y},\quad y\in [0,\sqrt{n}],
\end{align}
where $c,C>0$ are finite constants and the upper bound being true for any $y\geq 0$.
\eqref{equation:5.20}, \eqref{equation:5.19} and the upper bound in \eqref{equation:bound_tail_IBRW}, imply that there exists a constant $C>0$, such that \eqref{equation:tail_sum_IBRW} is bounded from above by
\begin{align}\label{equation:5.22}
\sum_{j=0}^{\lceil2(y-1)\rceil}\mathbb{P}\left(X^{*}_{N}\geq m_n+j\right)\mathbb{P}\left(X^{*,\prime}_{N}\geq m_n+2y-(j+1)\right)+ 2\mathbb{P}\left(X^{*}_{N}\geq m_n+2y\right)
\leq C(1+y)^4e^{-4y}.
\end{align}
\begin{prop}\label{proposition:8.2}
Let $x\in \mathbb{Z},$ $F^n_{n-s}(x)\coloneqq |\{u\in V_N:\, X^n_u(n-s)-2\log(2)(n-s\sigma_{max}^2) + \frac{\lambda n -s}{\lambda n} \frac{\log(n)}{4}+[-x-1,-x] \}|,$  and assume that $s\leq \lambda n$. Then, there is a universal constant $C>0$, such that for all $x\in \mathbb{Z}$,
\begin{align}\label{equation:expected_num_F^n_n(x)}
\mathbb{E}\left[F^n_{n-s}(x)\right]\leq C \exp\left[2\log(2)s(\sigma_{max}^2-1)+2x-\frac{\left(x+\log n\frac{\lambda n -s}{4\lambda n}\right)^2}{2\log(2)(n-s\sigma_{max}^2)}\right].
\end{align} 
Further, for any $u>-x$ satisfying $0<x+u<\sqrt{n/2}$, we have
\begin{align}
\mathbb{P}\left(F^n_{n-s}(x)\geq \exp\left(2\log(2)s(\sigma_{max}^2-1)+2(x+u)\right)\right)\leq C \exp\left(-2u\right).
\end{align}
\end{prop}
Note that the assumption $s\leq \lambda n$ poses no restriction, as for $s>\lambda n$, the BRW runs at speed zero, and thus, for any $v\in V_N$, we have $X^N_v(n-s)=0$.
\begin{proof}
We begin with the proof of \eqref{equation:expected_num_F^n_n(x)}. Noting that there are $4^{n-s}$ distinct particles at time $n-s$ and using a Gaussian tail estimate, it holds that
\begin{align}\label{equation:5.25}
\mathbb{E}\left[F^n_{n-s}(x)\right]
&=4^{n-s}\mathbb{P}(X^N_u(n-s)-2\log(2)(n-s\sigma_{max}^2)+\frac{\lambda n -s}{\lambda n} \frac{\log(n)}{4}\in [-x-1,-x])\nonumber \\ &
\leq \tilde{C} \frac{4^{n-s}}{\sqrt{2\pi \log(2)\sigma_{max}^2(\lambda n -s)}}\exp\left[-\frac{\left(2\log(2)(n-s\sigma_{max}^2)-\frac{\lambda n -s}{\lambda n} \frac{\log(n)}{4}-x \right)^2}{2\log(2)(n-s\sigma_{max}^2)}\right]\nonumber\\
& \leq C \exp\left[2\log(2)s(\sigma_{max}^2-1)\right]\exp\left[2x-\frac{\left(x+\frac{\lambda n -s}{\lambda n} \frac{\log(n)}{4}\right)^2}{2\log(2)(n-s\sigma_{max}^2)}\right].
\end{align}
The second statement follows using Markov's inequality and \eqref{equation:5.25}, i.e.
\begin{align}
\mathbb{P}\left(F^n_{n-s}(x)\geq \exp\left(2\log(2)s(\sigma_{max}^2-1)+2(x+u)\right)\right)
\leq \frac{ \mathbb{E}\left[F^n_{n-s}(x)\right]}{\exp\left(2\log(2)s(\sigma_{max}^2-1)+2(x+u)\right)}
\leq C e^{-2u}.
\end{align}
\end{proof}
\end{comment}
Write $u \underset{j}{\sim} v$, for $u,v \in V_N$, if $j$ is the largest integer such that $\mathcal{BD}_{n-j}(u)\cap \mathcal{BD}_{n-j}(v)\neq \emptyset$, i.e. in the language of BRW the ``splitting-time'' of $u$ and $v$ is $j$.
In the following proposition, we determine the position of extremal particles of an inhomogeneous BRW at the times when its variance changes. This is a direct consequence of \cite[Proposition 2.1]{MR3164771} in the weakly-correlated regime of variable speed BBM. Set $i(t,n)\coloneqq t\wedge (n-t)$.
\begin{proof}[Proof of the upper bound of \autoref{lemma:boundonexpofsumofmbrw}]
	\eqref{equation:5.38} allows to apply Sudakov-Fernique which, in combination with \eqref{corollary:upbound_prob_maxsum_BRW_statement3} in \autoref{corollary:upbound_prob_maxsum_BRW}, yields
	\begin{align}
	\mathbbm{E}\left[\tilde{S}^{*}_N\right]\leq 2m_n-c_1 \log \log r +\tilde{C}.
	\end{align}
	This concludes the proof of the upper bound of \autoref{lemma:boundonexpofsumofmbrw}.
\end{proof}
Let $\tilde{S}^{\diamond}_{N,r}=\max\{\tilde{S}^N_u(n)-\tilde{S}^N_u(2)+\tilde{S}^N_v(n)-\tilde{S}^N_v(2):u,v\in (N/4,N/4)+V_{N/2},r \leq \|u-v\|_2 \leq N/r \}$.
In order to prove the lower bound in \autoref{lemma:boundonexpofsumofmbrw}, we need the following proposition.
\begin{prop}\label{proposition:lb_prob_cutmaxsum_MBRW}
	There are constants $c_1,c_2>0$, such that for all $r\geq 1$ and sufficiently large $N\in \mathbbm{N}$,
	\begin{align}
	\mathbbm{P}\left(\tilde{S}^{\diamond}_{N,r}\geq 2m_n-c_1 \log\log r\right)\geq c_2.
	\end{align}
	\begin{proof}
		We may assume that $N\gg r$, in particular such that $\log_2 r /\log N \in (0,\lambda_1)$.
		By translation invariance of the 2d DGFF, we may consider $V_N$ as being centred at the origin. First, one gains additional independence of the MIBRW by leaving away the first $\log_2(r)+1$ contributions, i.e. decompose
		\begin{align}\label{equation:4.21}
		\tilde{S}^N_v&= \sum_{k=0}^{n-\log_2(r)-1}\sum_{B \in \mathcal{B}_k(v)}2^{-k}\sqrt{\log(2)}\sigma\left(\frac{n-k}{n}\right)b^N_{k,B}+\sum_{k=n-\log_2(r)}^{n}\sum_{B \in \mathcal{B}_k(v)} 2^{-k}\sqrt{\log(2)}\sigma\left(\frac{n-k}{n}\right)b^{N}_{k,B}\nonumber\\&\equiv \hat{S}^N_v+Y^N_v,
		\end{align}
		where $\{b^N_{k,B}\}_{k,B}$ is a family of independent standard Gaussian random variables. Furthermore, let $A_{n,r}= V_N \cap \left(\frac{N}{r}\mathbbm{Z}\right)^2.$
		For each $x\in A_{n,r}$, denote by $V_{N,r}(x)$ the $\mathbbm{Z}^2$-box centred at x of side length $\frac{N}{2r}$. $y\in A_{n,r}$ is a ``right neighbour'' of $x\in A_{n,r}$, if $y_1=x_1+N/r$ and $y_2=x_2$. In this case, write $y=x_R$.
		For $x\in A_{n,r}$, set
		\begin{align}
		S^{*}_{N,r,x}\coloneqq \max_{v \in V_{N,r}(x)} \hat{S}^N_{v}.
		\end{align}
		As $V_{N,r}^o(x) \cap V^o_{N,r}(y)=\emptyset$, for $x\neq y \in A_{r,n}$, it holds that $\{S^{*}_{N,r,x}\}_{x\in A_{n,r}}$ form an i.i.d. family of random variables.
		By \autoref{lemma:localization_MIBRW}, for $v\in V_N$ with $\tilde{S}^N_v\geq m_n-d$, we have $Y^N_v-2\log(2)\mathcal{I}_{\sigma^2}\left(\frac{\log_2(r)}{n}\right)n\in [-i^\gamma(\log_2(r),n),i^\gamma(\log_2(r),n)]$. By Gaussian comparison and \cite[Theorem~1.3]{MR2243875}, we know, with high probability, that there are $r^{2(1-\sigma_{1}^2)}$ many $x\in A_{r,n}$ such that $Y^N_x\geq 2\log(2)\mathcal{I}_{\sigma^2}\left(\frac{\log_2(r)}{n}\right)n$. Furthermore, $\mathrm{Var}\left[Y^N_u-Y^N_x\right]\leq C$, for $u \in V_{N,r}(x)$ from the inner quarter. Moreover, $\left\{\hat{S}^N_v\right\}_{v\in V_{N,r}(x)}$ and $\left\{\hat{S}^N_v\right\}_{v\in V_{N,r}(x)}$ are independent for $x\neq y \in A_{r,n}$. Combining these two observations with tightness of $\max_{v \in V_N} \tilde{S}^N_v- m_n$, there is a function $g:\mathbb{R} \mapsto \mathbb{R}$, satisfying $g(c)> 1/2 $ as $c\rightarrow \infty$, and such that
		\begin{align}\label{eq:uniformlb1}
		\mathbbm{P}\left(S^{*}_{N,r,x}\geq 2\log(2)\mathcal{I}_{\sigma^2}\left(\frac{\log_2(r)}{n},1\right)n-\frac{\log(n-\log_2(r))}{4}-c\right)
		\geq e^{2\log(2)\log_2(r)(\sigma_{1}^2-1)}g(c).
		\end{align}
		Let $\xi^{*}_{x,N}\in V_{N,r}(x)$ be such that $S^{*}_{N,r,x}=\hat{S}^{N}_{\xi^{*}_{x,N}}$ and set
		\begin{align}\label{equation:5.48}
		M_{N,r,c}\coloneqq \left\{x\in A_{n,r}:  S^{*}_{N,r,x}, S^{*}_{N,r,x_{R}}\geq2\log(2)\mathcal{I}_{\sigma^2}\left(\frac{\log_2(r)}{n},1\right)n-\frac{\log(n-\log_2(r))}{4}-c\right\}.
		\end{align}
		By independence of the two maxima in \eqref{equation:5.48} and by \eqref{eq:uniformlb1}, there is a constant $c>0$, such that
		\begin{align}
		\mathbbm{P}\left(|M_{N,r,c}|\geq\frac{r^{2\sigma_1^2}}{4}\right)\geq g(c)> \frac{1}{4}.
		\end{align}
		Next, we control $Y^N_v$ defined in \eqref{equation:4.21}.
		Set
		\begin{align}
		Z^N_x= Y^{N}_{\xi^{*}_{x,N}}+Y^{N}_{\xi^{*}_{x_R,N}},\quad \text{for } x\in A_{n,r}.
		\end{align}
		For $x,y\in A_{n,r}$ and conditioning on $\mathcal{F}_{N,r}=\sigma\left(\{\xi^{*}_{x,N} \}_{x\in A_{n,r}} \right)$, we have using \autoref{lemma:cov_comp} $i.$,
		\begin{align}
		\bigg| \mathbbm{E}&\left[Z^N_x Z^N_y|\mathcal{F}_{N,r} \right]-4\log(2) \sum_{i=1}^{M}\sigma_i^2\left[n\nabla \lambda_i \mathbbm{1}_{\log_2(r)-\log_+(d^N(x,y)/(N/r))\geq \lambda_i n} \right.\qquad\qquad\qquad\qquad\qquad\nonumber\\
		+&\left. \left(\log_2(r)-\log_{+}\left(\frac{d^N(x,y)}{N/r}\right)-\lambda_{i-1} \right)n\mathbbm{1}_{\lambda_{i-1}n<\log_2(r)-\log_{+}(d^N(x,y)/(N/r))<\lambda_i n} \right]\bigg| \leq C, 
		\end{align}
		where $C>0$ is a constant, independent of $N$ and $r$. On the event $|M_{N,r,c}|\geq r^{2\sigma_1^2}/4$, $Z^*_N=\max_{x\in A_{n,r}} Z^N_x$ can be lower bounded by twice the maximum of a MIBRW of $\lceil2\log 2 \log_2(r) \sigma_1^2 -\log 4\rceil$ generations and variance parameter $1$. This follows using Slepian's lemma, as variances of the two processes match but correlations in the MIBRW are strictly larger, as points on the underlying grid of the associated MIBRW have to be neighbouring, which is not necessarily true for particles in $M_{N,r,c}$. Thus, on the event $|M_{N,r,c}|\geq r^{2\sigma_1^2}/4$, and using \cite[Proposition~5.1]{MR2846636}, there are constants $\tilde{c},c_3>0$, independent of $N$ and $r$, such that
		\begin{align}
		\mathbbm{P}\left(Z^{*}_N\geq 2\left(2\log(2)\sigma_1^2 \log_2 r -\frac{3\log(\sigma_1^2\log_2 r)}{4}\right)-c_3 |\mathcal{F}_{N,r}\right)\geq \tilde{c}.
		\end{align}
		This allows to combine the two steps. Let $x^{*}_N \in M_{N,r,c}$ be the (unique) element such that $Z^{*}_N=Z^N_{x^{*}_N}.$ On the event $|M_{N,r,c}|\geq r^{2\sigma_1^2}/4$, which holds with probability $g(c)$, we have
		\begin{align}
		\tilde{S}^{\diamond}_{N,r}\geq Z^N_{x^{*}_N}+2\left[2\log(2)\mathcal{I}\left(\frac{\log_2 r}{n},1\right)n-\frac{3\log(n-\log_2 r)}{4}\right]-2c.
		\end{align}
		Thus, with probability at least $c_2\coloneqq g(c)\cdot \tilde{c}$, there is a constant $c_1>0$, such that
		\begin{align}
		\tilde{S}^{\diamond}_{N,r}\geq 2m_n-c_1\log \log r,
		\end{align}
		which concludes the proof of \autoref{proposition:lb_prob_cutmaxsum_MBRW}.
	\end{proof}
\end{prop}
\begin{proof}[Proof of the lower bound in \autoref{lemma:boundonexpofsumofmbrw}]
	Fix some integer $C=2^c>1$ and consider the MIBRW $\tilde{S}^{N,C}_v=\tilde{S}^{NC}_v(n-c-2)$ in a box $V_{NC}$ with levels up to $\log_2 \left( \frac{N}{4}\right)$, i.e. at least the last $c+2$ steps are not taken. Let $\overset{\diamond}{S}_{N,C,r}$ be defined in analogy to $\overset{\diamond}{S}_{N,r}$ in \eqref{equation:5.3}, simply replacing $\tilde{S}^N_v$ by $\tilde{S}^{N,C}_v$ and $N$ by $CN$.
	By independence of the field in sub-boxes of side $N/4$ with pairwise distance of at least $N/2$, we get using \autoref{proposition:lb_prob_cutmaxsum_MBRW},
	\begin{align}
	\mathbbm{P}\left(\overset{\diamond}{S}_{N,C,r}\geq 2 \mathbb{E}\left[\max_{v\in V_{CN}}\tilde{S}^{N,C}_v\right]-c_1\log\log r \right)\geq 1-(1-c_2)^{C^2/2}.
	\end{align}
	Adding the missing $c+2$ steps and a Gaussian estimate, one obtains
	\begin{align}\label{eq:inequality1_ProofLemma5.1}
	\mathbbm{P}\left(\overset{\diamond}{S}_{NC,r}\geq 2 m_{n+\log_2 (c)}-c_1\log\log r-y \right)\geq 1-(1-c_2)^{C^2/2}-c_3e^{-c_4y^2/c}.
	\end{align}
	In \eqref{eq:inequality1_ProofLemma5.1}, renaming $NC$ as $N$, choosing $y=c_5c$ and summing over $c\geq 0$,  concludes the proof of the lower bound in \autoref{lemma:boundonexpofsumofmbrw}, i.e. one obtains $\mathbbm{E}\left[\overset{\diamond}{S}_{N,r} \right]\geq 2m_n-c_6\log\log r.$
\end{proof}
\begin{cor}\label{corollary:bound_expectation_maxsum_IGFF}
	There are constants $c_1, c_2>0$ and $C>0$, such that, for all $r\geq 1$ and $N\in \mathbbm{N}$, sufficiently large,
	\begin{align}
	2 m_n -c_2 \log\log r -C \leq \mathbbm{E}\left[\overset{\diamond}{\psi}_{N,r} \right]\leq 2 m_n - c_1 \log\log r + C.
	\end{align}
	\begin{proof}
		This follows from \autoref{proposition:comparison_to_maxsum_MIBRW} together with \autoref{lemma:boundonexpofsumofmbrw}.
	\end{proof}
\end{cor}
\begin{comment}
\begin{lemma}
There exists a constant $c>0$, such that if for some $\epsilon,\lambda>0$ and $N,r\in \mathbbm{N}$,
\begin{align}
\mathbbm{P}\left(\exists u,v\in V_N: \, r\leq \|u-v\|_2\leq \frac{N}{r}\text{ and } \psi^N_u,\psi^N_v\geq m_n-\lambda\right)\geq \epsilon,
\end{align}
then for any $\delta>0$, setting $C(\delta,\epsilon)= 2\log(\delta) /\log(1-\epsilon)$ and $\gamma= c(\sqrt{\log(C(\delta,\epsilon))}/\delta)$, and for any $N^{'}=2^{n'}$ with $n' = \min\{m:\,2^m\geq C(\delta,\epsilon)N\}$, we have
\begin{align}
\mathbbm{P}\left(\overset{\diamond}{\psi}_{N,r}\geq 2 m_n-2\lambda-\gamma\right)\geq 1-\delta.
\end{align}
\end{lemma}
\end{comment}
\begin{lemma}\label{lemma:tightness_maximalsum}
	The sequence $\left\{\left( \overset{\diamond}{\psi}_{N,r}-\mathbbm{E}\left[\overset{\diamond}{\psi}_{N,r} \right] \right)/(\log\log r)\right\}_{N\in \mathbbm{N},r\in \{0,\dotsc,N\} }$ is tight.
	Moreover, there exists a constant $C>0$ such that with high probability, for all $N\in \mathbbm{N}$,
	\begin{align}
	\left|\overset{\diamond}{\psi}_{N,r}-\mathbbm{E}\left[\overset{\diamond}{\psi}_{N,r} \right]\right| \leq C \log\log r.
	\end{align}
	\begin{proof}
		Consider $V_{2N}$ and partition it into four translations of $V_N$, denoted by $V^{1}_N,V^{2}_N,V^{3}_N,V^{4}_N$. Let $\{\psi^{N,i}_v \}_{v\in V_N^i}$, for $i=1,\dotsc,4$, be four independent scale-inhomogeneous DGFFs.
		Define another Gaussian field on $V_{2N}$, $\{\hat{\psi}^{2N}_v\}_{v\in V_{2N}}$, by setting
		\begin{align}
		\hat{\psi}^{2N}_v=\psi^{N,i}_v,\qquad \text{for }v\in V_N^i.
		\end{align}
		As $\mathbbm{E}\left[\hat{\psi}^{\diamond}_{2N,r}\right]\geq \mathbbm{E}\left[\max\left(\overset{\diamond}{\psi}_{N,r,1},\overset{\diamond}{\psi}_{N,r,2} \right)\right]$, \autoref{corollary:bound_expectation_maxsum_IGFF} implies that
		\begin{align}
		\mathbbm{E}\left[\hat{\psi}^{\diamond}_{2N,r}\right]\geq 2m_n-c_2\log \log r-C.
		\end{align}
		For the upper bound one can use independence of $\psi^{N,i}_v$ on $V_N^{1},\dotsc, V_N^4$, and then for each field apply \autoref{corollary:bound_expectation_maxsum_IGFF}. Due to four independent of such Gaussian fields, one gets an additional constant, i.e. it holds that
		\begin{align}\label{equation:5.63}
		2m_n-c_2\log \log r-C\leq \mathbbm{E}\left[\hat{\psi}^{\diamond}_{2N,r}\right]\leq 2 m_n -c_1\log\log r +C.
		\end{align}
		With \eqref{equation:5.63},  $\mathbbm{E}\left[\hat{\psi}^{\diamond}_{2N,r}\right]\geq \mathbbm{E}\left[\max\left(\overset{\diamond}{\psi}_{N,r,1},\overset{\diamond}{\psi}_{N,r,2} \right)\right]$ and the fact that $|a-b|=2(a\vee b)-a-b,$ it follows
		\begin{align}
		\mathbbm{E}\left[\left|\overset{\diamond}{\psi}_{N,r,1}-\overset{\diamond}{\psi}_{N,r,2}\right| \right]\leq 2 \left(\mathbbm{E}\left[\hat{\psi}^{\diamond}_{2N,r}\right]- \mathbbm{E}\left[\overset{\diamond}{\psi}_{N,r} \right] \right)\leq C^{'}\log\log r+C,
		\end{align}
		which concludes the proof of \autoref{lemma:tightness_maximalsum}.
	\end{proof}
\end{lemma}
\begin{rem}
	We want to remark that at this stage it is possible to give an alternative proof of \cite[Theorem~2.2]{paper2} following  the proof of ... .
\end{rem}
\begin{proof}[Proof of \autoref{thm:prob_dist_maximalparticles}]
	Suppose that the claim in \autoref{thm:prob_dist_maximalparticles} is false. Then, for any constant $c>0$, there is an $\epsilon>0$ and a subsequence $\{r_k\}_{k\in \mathbbm{N}}$, such that for all $k\in \mathbbm{N}$,
	\begin{align}\label{eq:assumption_pf_maxparticles}
	\lim\limits_{N\rightarrow \infty}\mathbbm{P}\left(\exists u,v:\, r_k\leq \|u-v\|\leq N/r_k,\,\psi^N_u,\psi^N_v\geq m_n-c\log\log r_k \right)>\epsilon.
	\end{align}
	Fix $\delta>0$ and consider $N^{'}=2^k N$, where $k\in \mathbbm{N}$ is selected later in the proof. Partition $V_{N^{'}}$ into $2^{2k}$ disjoint boxes of side N, denoted by $V_N^1,\dotsc,V_N^{4^k}$.
	Let $\{\hat{\psi}^{N^{'}}_v\}_{v \in V_{N^{'}}}$ be defined by
	\begin{align}
	\hat{\psi}^{N^{'}}_v=\psi^{N,i}_v \qquad \text{ for } v \in V_N^i,
	\end{align}
	where $\{\psi^{N,i}_v \}_{v \in V_N^i}$ are i.i.d. scale-inhomogeneous DGFFs. As in the proof of \autoref{lemma:tightness_maximalsum}, \autoref{corollary:bound_expectation_maxsum_IGFF} holds for $\{\hat{\psi}^{N^{'}}_v\}_{v \in V_{N^{'}}}$ with an increased constant $C>0$, i.e.
	\begin{align}\label{equation:contradiction_pf_position_maxparticles}
	2m_n-c_2\log\log r -C\leq \mathbbm{E}\left[\hat{\psi}^{\diamond}_{N^{'},r} \right]\leq 2 m_n-c_1 \log\log r +C,
	\end{align}
	where $c_1,c_2>0$ are fixed constants and $C=C(k)>0$, a constant depending on $k$.
	Next, we derive a contradiction to \eqref{equation:contradiction_pf_position_maxparticles}. Set $z_{N,r}=2m_n-c\log\log r,\, Z_{N,r}=\left(\hat{\psi}^{\diamond}_{N{'},r}-z_{N,r} \right)_{-}$ and $Y^i_{N,r}=\left(\psi^{\diamond,i}_{N,r} -z_{N,r} \right)_{-}$.  \eqref{eq:assumption_pf_maxparticles} implies
	\begin{align}\label{eq:1_pf_maxparticles}
	\lim\limits_{N\rightarrow\infty}\mathbbm{P}\left(Y^1_{N,r_k}>0\right)\leq 1-\epsilon \qquad \forall k\in \mathbbm{N}.
	\end{align}
	Moreover, by \autoref{corollary:bound_expectation_maxsum_IGFF} and \autoref{lemma:tightness_maximalsum} there is a constant $C^{'}>0$ and an integer $r_0$, such that, for all $r\geq r_0$ and $N\in \mathbbm{N}$,
	\begin{align}\label{eq:2_pf_maxparticles}
	\mathbbm{E}\left[Y^1_{N,r} \right]\leq C^{'}\log\log r.
	\end{align}
	As, $Z_{N,r}\leq \min\limits_{1\leq i\leq 2^{2k}}Y^i_{N,r}$ and $\{Y^i_{N,r}\}_{1\leq i\leq 2^{2k}}$ are i.i.d. random variables, we have
	\begin{align}\label{equation:5.71}
	\mathbbm{E}\left[Z_{N,r_k} \right]&\leq \int_{0}^{\infty}\mathbbm{P}\left(Y^1_{N,r_k}>y \right)^{2^{2k}}\mathrm{d}y\leq (1-\epsilon)^{2^{2k}-1}\int_{0}^{\infty}\mathbbm{P}\left(Y^1_{N,r_k}>y \right)\mathrm{d}y\leq (1-\epsilon)^{2^{2k}-1}\mathbbm{E}\left[Y^1_{N,r_k} \right],
	\end{align}
	where we used \eqref{eq:1_pf_maxparticles} in the last inequality.
	Combining \eqref{equation:5.71} with \eqref{eq:2_pf_maxparticles}, one obtains for all $k,N \in \mathbbm{N}$,
	\begin{align}
	\mathbbm{E}\left[Z_{N,r_k} \right]\leq (1-\epsilon)^{2^{2k}-1}C^{'}\log\log r_k.
	\end{align}
	Choosing $c=c_1/4$ in \eqref{eq:assumption_pf_maxparticles} and $k$ such that $(1-\epsilon)^{2^{2k}}C^{'}\leq c_1/4$, allows to conclude that, for all $k\in \mathbbm{N}$ and $N\geq N_k$, for some $N_k\in 
	\mathbb{N}$ depending on $k$, it holds 
	\begin{align}\label{equation:5.66}
	\mathbbm{E}\left[\hat{\psi}^{\diamond}_{N^{'},r_k} \right]\geq 2m_n-c_1 \log\log r_k/2.
	\end{align}
	Letting first $N\rightarrow \infty$ and then $k\rightarrow\infty$, \eqref{equation:5.66} contradicts the upper bound in \eqref{equation:contradiction_pf_position_maxparticles} and thus, it also contradicts \eqref{eq:assumption_pf_maxparticles}, which concludes the proof of \autoref{thm:prob_dist_maximalparticles}.
\end{proof}
\par
For the proof of \autoref{theorem:distributional_invariance}, we refer the reader to the proof by Biskup and Louidor in the case of the DGFF (\cite[Theorem~3.1]{MR3509015}). This is possible, as we are able to provide for any ingredient used in their proof a corresponding one in the case of $(\sigma,\lambda)-$DGFF. With \autoref{theorem:size_of_level_sets}, we provide the last necessary property, i.e. a strong notion of tightness of extreme level sets. As in the proof of the separation of local extremes, i.e. of \autoref{theorem:separation_local_extremes}, the key object we need to study is the maximal sum of a fixed number of the field values, i.e.
\begin{align}
S_{l,N}=S_{l,N}(\psi)\coloneqq \max \left\{\sum_{v\in U} \psi_v: U\subset V_N,\, |U|=l \right\}.
\end{align}
The proof is based on the following two lemmas.
	\begin{lemma}\label{lemma:dist_invariance_1}
		There are constants $c_1,c_2\in (0,\infty)$ such that for all $\lambda>0,\,l\geq 1$ and $N\geq 1$,
		\begin{align}
			\mathbb{P}\left(S_{l,N}(\psi^N)<l(m_N-\lambda)\right)>c_1 -c_2 \frac{\lambda}{\log l}.
		\end{align}
	\end{lemma}

\begin{lemma}\label{lemma:dist_invariance_2}
	There are constants $c_3,c_4 \in (0,\infty)$ such that the following is true for all $\epsilon, \delta>0$ sufficiently small: Set $\sigma \coloneqq \epsilon^{-1}\log(1/\delta)$ and, for given $\lambda>0$ and $l\in \mathbb{N}$, let
	\begin{align}
		\lambda^{\prime}\coloneqq \lambda + c_4 \left(1+\log \sigma + \sqrt{\log(l/\delta)\log \sigma}\right).
	\end{align}
	If for some $N^{\prime}\geq 1$
	\begin{align}\label{equation:eq1_2nd_lemma_dist_inv}
		\mathbb{P}\left(S_{l,N^{\prime}}(\psi^{N^\prime})<l(m_{N^\prime}-\lambda^{\prime}) \right)>\delta,
	\end{align}
	then
	\begin{align}
		\mathbb{P}\left(|\Gamma_N(\lambda)|>l \right)<\epsilon
	\end{align}
	holds for all $N\in \mathbb{N}$ with
	\begin{align}
		N\leq c_3 \sigma^{-1/2}N^{\prime}.
	\end{align}
\end{lemma}

Before we provide the technical proofs, let us deduce \autoref{theorem:size_of_level_sets} first. As the proof provided in \cite{MR3509015} is neat and short, and since \autoref{lemma:dist_invariance_1} and \autoref{lemma:dist_invariance_2} provide the necessary conditions, we just copy it for the sake of completeness:
Let $c_1,c_2$ be the constants from \autoref{lemma:dist_invariance_1}. Given $\lambda>1$ and $\kappa>1$, define $l\coloneqq \lceil e^{\kappa \lambda}\rceil$ and set $\epsilon \coloneqq e^{-\beta \kappa \lambda}$ for some $\beta \in (0,1)$ still to be determined later in the proof.
Fix $\delta\in (0,c_1)$ and let $\lambda^{\prime}$ as in \autoref{lemma:dist_invariance_2}. For $\beta>0$ sufficiently small, $\lambda>0$ and $\kappa \geq \kappa_0(\beta,\lambda)$ -- so that $\beta \kappa \lambda$ is large -- we have
\begin{align}
	\lambda^{\prime}\leq \lambda (1+ \tilde{c}_1 \sqrt{\beta}\kappa).
\end{align}
And so, $\lambda^{\prime}/\log l = \mathcal{O}\left(\sqrt{\beta}\right)+\mathcal{O}(\kappa^{-1})$. Choosing $\beta$ small and $\kappa$ large,
\begin{align}
	c_1-c_2 \frac{\lambda^{\prime}}{\log l}>\delta.
\end{align}
By \autoref{lemma:dist_invariance_1}, we have
\begin{align}
	\mathbb{P}\left(S_{l,N^{\prime}}(\psi^{N^\prime})<l(m_{N^\prime}-\lambda^\prime)\right)>\delta,
\end{align}
which allows us to apply \autoref{lemma:dist_invariance_2}, to deduce that
\begin{align}
	\mathbb{P}\left(|\Gamma_N(\lambda)|>e^{\kappa \lambda}\right)<e^{-\kappa \lambda},
\end{align}
holds for all $N\leq c_3 \sigma^{-1/2}N^\prime$. As $N^\prime$ was arbitrary, the claim holds for all $N\geq 1$.
In order to prove these, we still need two more Lemmata.
\begin{lemma}\label{lemma:dist_invariance_3}
	\begin{align}
		\mathbb{E}\left[S_{l,N}(\psi^N) \right]\leq l(m_N-c \log l).
	\end{align}
	\begin{proof}
		By \cite[Corollary~8.1]{bibid}, we have
		\begin{align}
			\mathbb{E}\left[S_{l,N}(\psi^N)\right]\leq \mathbb{E}\left[S_{l,2^k N}(R^{2^k N})\right],
		\end{align}
		where $\{R^N_v\}_{v\in V_N}$ is the associated time-inhomogeneous BRW as in \cite[Defintion~6.1]{bibid} and $k>0$ is a fixed, uniform integer. Therefore, it suffices to bound
		\begin{align}
			\mathbb{E}\left[S_{l,N}(R^N)\right].
		\end{align}
		Let $F_{n}(x)= |\{u\in V_N: R^N_u-2\log(2)n -\log(n)/4 \in [-x-1,-x]\}|$.
		By \cite[Proposition~8.2]{bibid},
		\begin{align}
			\mathbb{P}\left(F_n(x)\geq \exp(2 (x+u)) \right)\leq C \exp(-2u),
		\end{align}
		for any $u>-x$, so that $0<x+ u <\sqrt{n/2}.$
		In particular,
		\begin{align}\label{equation:pf_lemma_5.3_2}
			\mathbb{P}\left(F_n(\log(l/2)/4)\geq \exp( \log(l/2))\right)\leq C \exp(-\log(l/2)/2).
		\end{align}
		Now, we use the observation that
		\begin{align}\label{equation:pf_lemma_5.3_1}
			S_{l,N}(R^N)\leq l R^{*}_N-\frac{l \log(l)}{8}\mathbbm{1}_{F^{*}_{n,\log(l/2)/4}\leq l/2},
		\end{align}
		where $F^{*}_{n,x}= \cup_{i=m_N- R^{*}_N}^x F_n(i)$.
		We write
		\begin{align}\label{equation:pf_lemma_5.3_3}
			\mathbb{E}\left[S_{l,N}(R^N)\right]=\mathbb{E}\left[S_{l,N}(R^N)(\mathbbm{1}_{F^{*}_{n,\log(l/2)/4}\leq l/2} + \mathbbm{1}_{F^{*}_{n,\log(l/2)/4}> l/2} ) \right].
		\end{align}
		The first term, we can estimate using \eqref{equation:pf_lemma_5.3_1}, for the second, we use \eqref{equation:pf_lemma_5.3_2} along with an upper bound on the right-tail of the centred maximum by Mallein (cp. \cite[Theorem~4.1]{MR3361256}), i.e.
		\begin{align}
			\mathbb{P}\left(\max_{v \in V_N} R^N_v\geq m_N +x \right)\leq (1+x)\exp(-2x).
		\end{align}
		So, for the second term in \eqref{equation:pf_lemma_5.3_3}, we simply bound $S_{l,N}(R^N)$ by $l$ times the maximal particle on the second event, which yields as an upper bound
		\begin{align}
			\mathbb{E}\left[S_{l,N}(R^N) \mathbbm{1}_{F^{*}_{n,\log(l/2)/4}> l/2} \right]\leq C l  \exp(-\log(l/2)/2) \mathbb{E}\left[R^{*}_N\right]\leq \tilde{C} \sqrt{l} (m_N +\tilde{c})\leq l(m_N - c \log(l)),
		\end{align}
		for some constant $c>0$, once we pick $l$ sufficiently large.
		Altogether, there is a constant $c>0$ such that for all $N$ and $l$ sufficiently large,
		\begin{align}
			\mathbb{E}\left[S_{l,N}(\psi^N)\right]\leq l (m_N -c \log(l)).
		\end{align}
	\end{proof}
\end{lemma}
Analogously to \cite[Lemma~4.6]{MR3262484}, we have:
\begin{lemma}\label{lemma:dist_invariance_4}
	Let $\Xi_{N,r}\coloneqq \{(u,v)\in V_N\times V_N :\, r\leq |u-v|\leq N/r \}$. Then,
	\begin{align}\label{equation:DGFF_decomposed_mblocks}
		\mathbb{P}\left(\exists A \subset \Xi_{N,r}:\, |A|\geq \log r,\, (u,v)\in A\implies \psi^N_u+\psi^N_v\geq2( m_N- \lambda \log \log r) \right)
		\geq 1 - Ce^{-e^{c \lambda  \log \log r}}.
	\end{align}
	\begin{proof}
		We adapt the proof from Ding and Zeitouni which deals with the case of the DGFF (\cite[Lemma~4.6]{MR3262484}): Let
		$R=N(\log r)^{-\lambda /10}$, $l=N(\log r)^{-\lambda/100}$ and $o_i=(il, 2R)$ $1\leq i \leq M=(\log r)^{\lambda/100 }/2$ be the centres of boxes $C_i$ of side $R$. Further let $B_i\subset C_i$ boxes with the same centre $o_i$ of side length $R/8$. Next, we collect the boxes into $m=(\log r)^{\lambda/200}$ blocks, i.e. let $\mathcal{C}_i=\{C_j:\, (i-1)m<j<i m \}$ and $\mathcal{B}_i=\{B_j:\, (i-1)m<j<i m \}$. We can now consider our $(\sigma,\lambda)-$DGFF on each collection $\mathcal{C}_i$ for simplicity let $\mathcal{C}=\mathcal{C}_1$ and $\mathcal{B}=\mathcal{B}_1$, i.e. using Gibbs-Markov for the underlying DGFF $\{\phi^N_v\}_{v\in V_N}$ as in \eqref{equation:inhomogeneous_GM}, we have
		\begin{align}\label{equation:GM_B_C_V}
			\psi^{N}\overset{d}{=} \tilde{\psi}^{C}+\Phi^{N,C},
		\end{align}
		where $\{\tilde{\psi}^C_v\}_{v\in V_N}$ is a $(\sigma,\tilde{\lambda})-$DGFF on $C$ with slightly changed scale-parameters $\tilde{\lambda}_i,\, i=1,\dotsc, M$ and which is independent of the other Gaussian field $\{\Phi^{N,C}_{v}\}_{v\in V_N}$. The new scale parameters are chosen such that $[v]^N_{\lambda_i}=[v]^R_{\tilde{\lambda}_i}$ for $i=1,\dotsc, M$, i.e. we want that the boundaries of the boxes match, so that we sum over the same vertices, and so we set $[v]^R_0=V_N$. The centred Gaussian field $\{\Phi^{N,C}_{v}\}_{v\in V_N}$ is discrete harmonic as a weighted sum of discrete harmonics, which is a consequence of the Gibbs-Markov property and which also allows for the explicit representation
		\begin{align}\label{equation:scale_dep_disc_harmonic}
			\Phi^{N,C}_v=\sum_{i=1}^{M}\sigma_i \nabla \phi^{N,C}_v(\tilde{\lambda}_i)
			=\sum_{i=1}^{M}\sigma_i \left(\sum_{w\in [v]^R_{\tilde{\lambda}_i}}\mathbb{P}_v\left(S_{\tau_{\partial [v]^R_{\tilde{\lambda}_i}}=w }\right)  \phi^{N,C}_w - \sum_{w\in [v]^R_{\tilde{\lambda}_{i-1}}} \mathbb{P}_v\left(S_{\tau_{\partial [v]^R_{\tilde{\lambda}_{i-1}}}}=w\right) \phi^{N,C}_w \right),
		\end{align} 
		where $\{\phi^{N,C}_{v\in V_N} \}$ is the discrete harmonic extension of the DGFF $\{\phi^N_v\}_{v\in V_N}$ from the values in $V_N\setminus \text{clos}(C)$ to $C$. Here, we also assume, in order to avoid additional notation due to otherwise necessary case distinctions, that $N$ is so large, that $[v]^N_{\lambda_i}\subset C$ for $v\in B\subset C\subset V_N$.
		Let, $\xi_{B,1},\xi_{B,2}\in B$ such that
		\begin{align}
		\tilde{\psi}^C_{\xi_{B,1}}+\tilde{\psi}^C_{\xi_{B,2}}=\max_{u,v\in B\times B \cap \Xi_{N,r}}\tilde{\psi}^C_u+\tilde{\psi}^C_v.
		\end{align}
		Thus, by \cite[Corollary~8.3 and Lemma~8.3]{keylist} (ref. to  sum of two vertices of $(\sigma,\lambda)-$DGFF from convergence of the centred maximum paper), we obtain
		\begin{align}
		\mathbb{P}\left(\tilde{\psi}^C_{\xi_{B,1}}+\tilde{\psi}^C_{\xi_{B,2}w}\geq 2 m_N -\lambda \log \log r \right)\geq 1/4.
		\end{align}
		Let $W=\{ (\xi_{B,1},\xi_{B,2}):\,\tilde{\psi}^C_{\xi_{B,1}}+\tilde{\psi}^C_{\xi_{B,2}}\geq 2 m_N -\lambda \log \log r,  B\in \mathcal{B} \}.$ By independence and Gaussian concentration,
		\begin{align}\label{equation:5.16}
		\mathbb{P}\left(|W| \leq  m/8 \right)\leq e^{-cm}.
		\end{align}
		We still have to exclude that the second Gaussian field in \eqref{equation:GM_B_C_V} $\{\Phi^{N,C}_v +\Phi^{N,C}_w\}_{ (v,w) \in W}$, the modified harmonic extension, is too negative. Thus, consider
		$U\subset \cup_{B\in \mathcal{B}}B\times B$, $|U|\geq m/8$. With slight modifications of the proof of \cite[Lemma~4.7]{MR3262484} we will get just that. The modifications are needed, as we want to use the $(\sigma,\lambda)-$DGFF on boxes, which is why we use $C_i$ as boxes instead of discrete balls as done in \cite[Lemma~4.7]{MR3262484}. They do so, since the potential kernel on the circle is essentially constant and so the estimates are fairly easy, whereas on boxes, it changes up to bounded constant, depending on the geometric position on the box. However, as we will see this does not matter for the proof as it uses only upper bounds on the correlations up to multiplicative constants there. Our aim is to proof
		\begin{align}
			\mathrm{Var}\left[\Phi^{N,C}_v\right]\leq \mathcal{O}(\lambda \log \log r),\\
			\mathbb{E}\left[\Phi^{N,C}_u \Phi^{N,C}_v \right]\leq \mathcal{O}(\lambda \log \log r \sqrt{R/l}),
		\end{align}
		which allows us to deduce as in \cite[Lemma~4.7]{MR3262484}, since its proof essentially only uses these two estimates to employ Gaussian comparison and thereby obtain the claim.
		As mentioned, we still need to argue, why this bounds hold. When looking at \eqref{equation:scale_dep_disc_harmonic}, we see that the inner sums are harmonic averages of the discrete harmonic extension from the DGFF. In particular, the probabilities occuring are uniformly bounded by $c/N^{1-\lambda_i}$ (see below for an argument). This reduces our proof to uniformly bound the correlation of any two elements in the double sums, that we obtain when computing the correlation.
		We see, that for $v\in B\subset C$
		\begin{align}
			\mathrm{Var}\left[\Phi^{N,C}_v \right]\leq c M \max_{i\geq 1} \max_{w\in [v]^N_{\lambda_i}} \mathrm{Var}\left[\phi^{N,C}_w\right].
		\end{align}
		Now, for $N$ sufficiently large, we have that $[v]^N_{\lambda_i}$ is included in a box of side length $R/4$, for any $i=1,\dotsc, M$. Thus, as the Poisson kernel of Brownian motion on $(0,1)^2$ is bounded and by comparing it to the properly rescaled discrete harmonic measure \cite[Proposition~8.1.4]{MR2677157}, we see that
		\begin{align}
			\mathbb{P}_w\left(S_{\tau_{\partial C} }=z\right)\leq c/R,
		\end{align}
		for some uniform constant $c>0$ and any $w\in \partial [v]^N_{\lambda_i}$, $i=1,\dotsc, M$.
		Thus,
		\begin{align}
			\mathrm{Var}\left[\phi^{N,C}_w \right]\leq c/R^2\sum_{u,v\in \partial C} G_{V_N}(u,v).
		\end{align}
		Now, we need to estimate the sum of the Green kernel on the boundary of the box $C$. As we need only upper bounds of the above order, we can replace the sum by the sum over vertices on a circle with radius $\frac{2}{\pi}R$, which has exactly as many vertices as the original one. This allows us to map vertices from the boundary of the box onto the circle keeping neighbouring relations. Thus, for any two vertices $x,y$ on the boundary of the box, we have vertices $x^\prime, y^\prime$ on the circle, such that $\big|\log\|x-y\| -\log\|x^\prime -y^\prime\| \big|\leq c_1$, and so by \cite[add. text]{keylist},
		\begin{align}
			|G_{V_N} (x,y)- G_{V_N}(x^\prime, y^\prime)| \leq c_1 + O(1/N^2).
		\end{align} 
		Therefore, by adding a constantly bounded error, we may replace the Green kernel for particles on the boundary of the box by the same Green kernel evaluated for particles on the circle. This allows us to invoke \cite[]{MR3101848}, to obtain
		\begin{align}
			\mathrm{Var}\left[\phi^{N,C}_v \right]\leq O(\lambda \log \log r).
		\end{align}
		For the correlation term, we first reduce it as above to a uniform bound on the correlation of the discrete harmonic extension and in order to estimate this, we can follow the proof in \cite{MR3101848} (cp. \cite[(18)]{MR3101848}), which deals with the case of circles instead of boxes. For $u\in C_i$ and $v\in C_j$ with $i\neq j$, and first reducing the estimate to an estimate on the discrete harmonic extension of the DGFF on boxes, we arrive at
		\begin{align}
			\mathbb{E}\left[\phi^{N,C}_w \phi^{N,C}_{w^\prime} \right]&\leq O(1/R) \max_{x \in C_i} G_{V_N}(x,\partial C_j)
			\leq O(1/R)\max_{x\in C_i} \mathbb{P}_x\left(\tau_{\partial C_j }<\tau_{\partial V_N}\right) \max_{y \in \partial C_j}G_{V_N}(y,\partial C_j)\nonumber\\
			& \leq O(1/R) \max_{x\in C_i}\mathbb{P}_x\left(\tau_{\partial C_j }<\tau_{\partial V_N}\right) \max_{y \in \partial C_j} \sum_{z\in \partial C_j}G_{V_N}(y,z)
			\leq O(\lambda \log \log r) \max_{x \in C_i}\mathbb{P}_x\left(\tau_{\partial C_j }<\tau_{\partial V_N} \right),
		\end{align}
		provided $N$ and $\lambda$ are sufficiently large. Thus, we are left with bounding the last probability.
		Note, that in the proof of Jian Ding, he is dealing with circles, so that we cannot directly use his results. Therefore,
		\begin{lemma}\cite[cp. Lemma~2.6]{MR3101848}
			For any $i\neq j$ and $x\in C_i$, we have
			\begin{align}
				\mathbb{P}_x\left(\tau_{\partial C_j }<\tau_{\partial V_N} \right)\leq C \sqrt{R/l},
			\end{align}
			where $C>0$ is a universal constant.
			\begin{proof}
				Our strategy is to use \cite[Lemma~2.6]{MR3101848}: Therefore, note that our box $C_j$ has side length R. So a circle $D$ with the same centre and radius $\sqrt{2}R$ includes the box, that is $D\supset C_j$. Thus, $\tau_{\partial D}<\tau_{\partial C_j }$, and so by \cite[Lemma~2.6]{MR3101848}
				\begin{align}
					\mathbb{P}_x\left(\tau_{\partial C_j }<\tau_{\partial V_N}\right)\leq \mathbb{P}_x\left(\tau_{\partial D}<\tau_{\partial V_N} \right) \leq \tilde{C} \sqrt{2R/l}\leq C \sqrt{R/l}.
				\end{align}
			\end{proof}
		\end{lemma}
		 Thus, we have the necessary correlation estimates, to be able to carry out the same proof as in  \cite[Lemma~4.7]{MR3262484}, to obtain
		\begin{align}\label{equation:5.27}
		\mathbb{P}\left(\exists(u,v)\in U:\, \Phi^{N,C}_u + \Phi^{N,C}_v\leq 0\right) \leq Ce^{-c (\log r)^{c\lambda}}.
		\end{align}
		This allows us to finish the proof of \autoref{lemma:dist_invariance_4}.
		Using conditional independence and the previous two estimates \eqref{equation:5.16} and \eqref{equation:5.27}, we deduce,
		\begin{align}
		&\mathbb{P}\left(\max_{B \in \mathcal{B}} \max_{(u,v)\in B\times B \cap \Xi_{N,r}} \} \psi^N_u+\psi^N_v\geq2( m_N- \lambda \log \log r) \right) \nonumber\\&\quad
		\geq \mathbb{P}\left(|W|> m/8 \cap \{\exists (u,v)\in W:\, \Phi^{N,C}_u+ \Phi^{N,C}_v >0 \} \right)\nonumber\\&\quad
		\geq \mathbb{P}\left(|W|>m/8  \right) \mathbb{P}\left(\exists (u,v)\in U:\, \Phi^{N,C}_u +\Phi^{N,C}_v >0| |U|\geq m/8 \right)\nonumber\\&\quad \geq
		(1-e^{-cm})(1-Ce^{-c(\log r)^{c \lambda}})\geq 1 -Ce^{-e^{c \lambda  \log r}}.
		\end{align}
		We return to the consideration of the partitioning into $m$ blocks, i.e.  let $(\chi_{j,1},\chi_{j,2})\in \mathcal{B}_j \times \mathcal{B}_j \cap \Xi_{N,r}$, such that
		\begin{align}
			\psi^N_{\chi_{j,1}}+\psi^N_{\chi_{j,2}}= \max_{B\in \mathcal{B}_j}\max_{(u,v)\in B\times B \cap \Xi_{N,r}} \psi^N_u +\psi^N_v.
		\end{align}
		Further, let  $A=\{(\chi_{j,1},\chi_{j,2}):\, 1\leq j \leq M/m \}$. A union bound gives
		\begin{align}
			\mathbb{P}\left(\min_{(u,v)\in A} \psi^N_u +\psi^N_v\geq 2 m_N - \lambda \log \log r \right) \geq 1 - Ce^{-c \lambda \log r},
		\end{align}
		which implies the claim.
	\end{proof}
\end{lemma}
\begin{proof}[Proof of \autoref{lemma:dist_invariance_1}]
	As the proof of the analogue statement \cite{MR3509015} is based only on estimates that are analogue to \autoref{lemma:dist_invariance_3} and \autoref{lemma:dist_invariance_4}, we refer to their proof.
\end{proof}
\begin{proof}[Proof of \autoref{lemma:dist_invariance_2}]
	We follow and adjust the proof of \cite[Lemma~4.3]{MR3509015}: We assume the opposite holds. Fix $\epsilon, \delta>0$ small enough and suppose that for some $\lambda>0$ and $N,l\geq 1$
	\begin{align}
		\mathbb{P}\left(|\Gamma_N(\lambda)|>l\right)\geq \epsilon.
	\end{align}
	Trivially, this implies
	\begin{align}\label{equation:1_pf_lemma_dist_invariance_2}
		\mathbb{P}\left(S_{l,N}(\psi^{N})>l(m_N-\lambda)\right)\geq \epsilon.
	\end{align}
	Pick $\varrho \in (0,1)$ and set $N^{\prime \prime }\coloneqq \floor \varrho^{-1}N\rfloor$ and $N^\prime\coloneqq \lfloor \sqrt{\sigma}\varrho^{-2}N\rfloor$. Note, that by this choice, $N^\prime > N^{\prime \prime}$ and so we can identify inside $V_{N^\prime}$, $k\coloneqq (\lfloor N^\prime/ 4N^{\prime \prime}\rfloor)^2$ disjoint translates $V^i_{N^{\prime \prime }}$ of $V_{N^{\prime \prime}}$ that we additionally assume to be at least at distance 2 apart and at least $N^\prime/4$ away from the boundary of $V_{N^\prime}$. In each $V^i_{N^{\prime \prime}}$ we place a copy of $V_N$, denoted $V^i_N$ with the same centre.
	As a first step, we claim that for a $(\sigma,\lambda)-$DGFF $\psi^{N^{\prime\prime}}$ on $V_{N^{\prime \prime}}$, it holds
	\begin{align}
		\mathbb{P}\left(S_{l,N}(\psi^{N^{\prime \prime}})>l(m_N-\lambda)\right)\geq \epsilon/2.
	\end{align}
	We invoke as in the previous proof the Gibbs-Markov decomposition
	\begin{align}
		\psi^{N^{\prime \prime}}\overset{d}{=} \tilde{\psi}^N+ \Phi^{N^{\prime \prime},N},
	\end{align}
	where $\tilde{\psi}^N$ is a $(\sigma,\tilde{\lambda})-$DGFF with slightly different scale parameters as in  \eqref{equation:inhomogeneous_GM}. Note, that this choice means in words, that we cut off the smallest increment in order to keep the size of the larger increments, which essentially leads in our case of increasing variance to a larger effective variance of the new scale-dependent DGFF. In particular, it follows
	\begin{align}\label{equation:5.25}
		\{S_{l,N}(\psi^{N^{\prime \prime}})>l(m_N-\lambda)\} &\supset ( \{S_{l,N}(\tilde{\psi}^N)>l(m_N -\lambda) \}\cap \{\sum_{v\in U_{l,N}(\tilde{\psi}^N)} \Phi^{N^{\prime \prime}}_v \geq 0 \})\nonumber\\
		&\supset ( \{S_{l,N}(\psi^N)>l(m_N-\lambda) \}\cap \{\sum_{v\in U_{l,N}(\tilde{\psi}^N)} \Phi^{N^{\prime \prime}}_v \geq 0 \}).
	\end{align}
	As the field $\Phi^{N^{\prime \prime},N}$ is an independent mean zero Gaussian field, the last event can be separately bounded from below by $1/2$ and for the first, we may apply \eqref{equation:1_pf_lemma_dist_invariance_2}, and so
	\begin{align}\label{equation:SLN''_1}
		\mathbb{P}\left(S_{l,N}(\psi^{N^{\prime \prime}})>l(m_N-\lambda) \right)\geq \epsilon/2.
	\end{align}
	We now turn to the $(\sigma,\lambda)-$DGFF on the entire box $V_{N^\prime}$:
	Analogously to \eqref{equation:inhomogeneous_GM}, we may decompose using the Gibbs-Markov property of the DGFF,
	\begin{align}
		\psi^{N^\prime}\overset{d}{=} \tilde{\psi}^{N^{\prime \prime},i}+ \Phi^{N^\prime, N^{\prime \prime}}, \quad \text{on } V^i_{N^{\prime \prime}}.
	\end{align}
	Using the same reasoning as for \eqref{equation:5.25}, i.e. that the fields $\tilde{\psi}^{N^{\prime \prime },i}$ have larger effective variance and their variances are still strictly increasing, we deduce
	\begin{align}\label{equation:lb_SlN_1}
		\{S_{l,N}(\psi^{N^\prime})>l(m_{N^\prime}-a-b) \}
		\supset (\{ \max_{1\leq i \leq n}S_{l,N}(\psi^{N^{\prime \prime},i})>l(m_{N^\prime}-a) \} \cap \{\min_{x\in U_{l,N}(\psi^{N^{\prime \prime}, K(\psi^{N^\prime})})}\Phi^{N^\prime, N^{\prime \prime}}_x \geq -b \}),
	\end{align}
	where $K(\psi^{N^\prime})$ denotes the maximizing index of $S_{l,N}(\psi^{N^{\prime \prime},i})$.
	Using a union bound, $\mathrm{Var}\left[\Phi^{N^\prime, N^{\prime \prime}} \right]\leq C \log N^\prime / \log N^{\prime \prime}=\mathcal{O}(\log \sigma)$ and a classical Gaussian estimate \cite{gordon1941}, we can bound the second event in \eqref{equation:lb_SlN_1} by
	\begin{align}\label{equation:lb_Phi_-b_1}
		\mathbb{P}\left(\min_{x\in U_{l,N}(\psi^{N^{\prime \prime}, K(\psi^{N^\prime})})} \Phi^{N^\prime, N^{\prime \prime}}\leq -b \right)&=1- \mathbb{P}\left(\max_{x\in U_{l,N}(\psi^{N^{\prime \prime}, K(\psi^{N^\prime})})} \Phi^{N^\prime, N^{\prime \prime}}<b\ \right)
		\geq 1-l\, \mathbb{P}\left(\Phi^{N^\prime,N^{\prime \prime}}<b\right)\nonumber\\ &
		\geq 1-l e^{-c^2 b^2/(\log \sigma)}.
	\end{align}
	If we set $b\coloneqq c_4 \sqrt{ \log(l/\delta)/\log \sigma}$, with $c_4>0$ sufficiently large, the right hand side of \eqref{equation:lb_Phi_-b_1} is lower bounded by $1-\delta/2$ uniformly in $l$.
	For the first event in \eqref{equation:lb_SlN_1}, we set $a\coloneqq m_{N^\prime}-m_N+\lambda$ and use the estimate \eqref{equation:SLN''_1} and assume $\varrho>0$ to be sufficiently small, so that altogether
	\begin{align}
		\mathbb{P}\left(\max_{1\leq i \leq k} S_{l,N}(\psi^{N^{\prime \prime },i})>l(M_{N}-\lambda) \right)\geq 1-(1-\epsilon/2)^k\geq 1-\delta/2.
	\end{align}
	Using that $m_{N^\prime}-m_N \leq C \log \sigma$ for $\delta, \epsilon>0$ small, it follows that $\lambda^\prime>a+b$, and so we may deduce
	\begin{align}
		\mathbb{P}\left(S_{l,N^\prime}(\psi^{N^\prime})>l(m_{N^\prime}-\lambda^\prime) \right) \geq \mathbb{P}\left(S_{l,N^\prime}(\psi^{N^\prime})>l(m_{N^\prime}-a-b)\right)\geq 1-\delta.
	\end{align}
	This contradicts \eqref{equation:eq1_2nd_lemma_dist_inv}, which gives our claim.
\end{proof}		
	 \begin{comment}
	 	To see that one is able to do that kind of decomposition, follows from the Gibbs-Markov property of the DGFF. Note, that the scale-dependent DGFF is a weighted sum of differences of the DGFF conditioned on the values of certain particles. By (), this takes the form for a set $A\subset V_N$
	 	\begin{align}
	 	\phi^{N^\prime}_v(A)=\sum_{w\in \partial A} \mathbb{P}_v\left(S_{\tau_{\partial A}}=w\right)\phi^{N^\prime}_w\overset{d}{=} \sum_{w\in \partial A} \mathbb{P}_v\left(S_{\tau_{\partial A}}=w\right)\left(\phi^N_w+ \Phi^{N^{\prime},N}_w \right)\nonumber\\
	 	=\phi^N(A)+\Phi^{N^\prime,N}(A)
	 	\end{align}
	 	Now, the first field, can again be approximated by a time-inhomogeneous MBRW and the second one is a Gaussian field with uniformly bounded variance, for which we can apply the same standard Gaussian estimate.
	 	The corresponding scales $\tilde{\lambda}_i,\,i=1,\dotsc,M$ have to satisfy $(N^{\prime})^{1-\lambda_i}=N^{1-\tilde{\lambda}_i}$, and so
	 	\begin{align}
	 	\tilde{\lambda}_i=1-\frac{(1-\lambda_i) n}{n^\prime}.
	 	\end{align}
	 	The following might be working for this as well, but I think it is by far less elegant than the solution above.
	 	The 
	 	\begin{align}
	 	\psi^N \overset{d}{=} \tilde{\psi} + \sigma_1 \mathbb{E}\left[\phi^N | \sigma\left(\phi^N_w:w\in \partial \mathcal{C}\right) \right],
	 	\end{align}
	 	where $\tilde{\psi}=\sum_{i>1}\sigma_i \nabla \phi^N_v(\lambda_i)+ \sigma_1\left(\phi^N_v(\lambda_1)-\phi^N_v(\mathcal{C})\right).$ Note, that the second summand, i.e. the first increment, is now a modified increment. Nevertheless, we can deduce Lemma and Corollary fr sum of two particles as in previous paper, by replacing the MBRW in there by a slightly different MBRW which has a modified first increment. The analysis in the proofs for this process is not affected at all by this, since it is still of the form and the same structure, that is the proof goes through, as the covariance estimate compared is affected only by a constant shift (\cite[Lemma~A.4 and Lemma~A.5]{MR3541850}). Thus the argument via Gaussian comparison to a MBRW as in ... works just as well. The only thing we need to modify in the MBRW is the first scale which define as the first scale of the MBRW on the box $C$ with modified first scale parameter $\tilde{\lambda}_1= \lambda_1 /(1-\frac{\log \log r}{10 n})$
	 \end{comment}	
	

==> proof_dist_invariance.tex <==
We could just refer to Marek/Orens paper, as it uses nothing that we do not have... Giving the principle idea/heuristics is nevertheless a good idea...

Let $\psi^{\prime}$, $\psi^{\prime \prime}$ be two independent copies of the $(\sigma,\lambda)-$DGFF on $V_N$. Fix $t>0$ and write
\begin{align}
	&\hat{\psi}^{\prime}\coloneqq \sqrt{1-\frac{t}{const. \log N}}\psi^\prime &\,\text{and}\, &\hat{\psi}^{\prime \prime}\coloneqq \sqrt{\frac{t}{const. \log N}}\psi^{\prime \prime}.
\end{align}
Then,
\begin{align}\label{equation:field_as_sum_perturbation}
	\psi\coloneqq \hat{\psi}^{\prime}+\hat{\psi}^{\prime \prime}
\end{align}
has the law of the $(\sigma,\lambda)-$DGFF on $V_N$. We assume that both $\hat{\psi}^{\prime}$ and $\hat{\psi}^{\prime \prime}$ are realized on a common probability space and that $\psi$ is given by their sum, that is by \eqref{equation:field_as_sum_perturbation}. Further, let
\begin{align}
	\Theta_{N,r} \coloneqq \left\{v\in V_N: \psi_v=\max\limits_{w\in \Lambda_r(v)}\psi_w \right\}
\end{align}
be the set of $r-$local maxima of the field $\psi$. Then for any function $f:[0,1]^2\times\rightarrow [0,\infty)$,
\begin{align}
	<\eta_{N,r},f>=\sum\limits_{v\in \Theta_{N,r}} f\left(v/N,\psi_v - m_N\right).
\end{align}
As we are working with the vague topology, our test functions will be compactly supported, and so if $f$ has in addition compact support, we may reduce the sum further to $\sum\limits_{v\in \Theta_{N,r}\cap \Gamma_N(\lambda)}f\left(v/N,\psi_v- m_N\right)$ for sufficiently large $\lambda$.
\begin{lemma}\cite[Lemma~4.4]{MR3509015}\label{lemma:reduction_to_fixed_r}
	Let $f:[0,1]^2\times \mathbb{R}\rightarrow [0,\infty)$ be measurable with compact support. Then for any $r_N\rightarrow \infty$ with $r_N/N\rightarrow \infty$,
	\begin{align}
		\lim\limits_{r\rightarrow \infty}\limsup\limits_{N\rightarrow \infty} \mathbb{P}\left(<\eta_{N,r_N},f>\neq <\eta_{N,r},f> \right)=0.
	\end{align}
\end{lemma}
For the proof we refer to \cite{MR3509015}, as it only uses the analogue statement of \autoref{theorem:separation_local_extremes} in the case of the DGFF. \autoref{lemma:reduction_to_fixed_r} allows us to work with a fixed $r>0$ instead of $r_N$.
The next proposition allows us to replace the positions of local extremes of the original field, we those of the "perturbed one".
\begin{prop}\label{proposition:perturbation_asymptotically_correct_local_maxima}
	Let $f:[0,1]^2\times \mathbb{R}\rightarrow [0,\infty)$ be continuous with compact support. Then for any $\epsilon>0$,
	\begin{align}
		\lim\limits_{r\rightarrow \infty}\limsup\limits_{N\rightarrow \infty}\mathbb{P}\left(|\sum\limits_{x\in\Theta_{N,r}}f\left(x/N,\psi^N_x - m_N \right)-\sum\limits_{x\in\Theta^{\prime}_{N,r}}f\left(x/N,\psi^N_x-m_N\right) |>\epsilon \right)=0.
	\end{align}
\end{prop}
The stuff here will follow completely analogously as in Mareks/Orens paper, as their proofs are based on Gaussian interpolation along with estimates that are available for the $(\sigma,\lambda)-$DGFF as well. We should think about essentially copying their proofs or just refering to theirs and saying that one just needs to replace the estimates and constants... as there is no essential new input, this might be a good option to keep the proof short.

==> proof_poisson_limit.tex <==
\begin{proof}[Proof of \autoref{theorem:poisson_limit_law}]
	I think, that we can basically cite Marek and Oren's paper. Their proof/statement is formulated in such a general way, that we can just use it, once having the distributional invariance.
\end{proof}
